A Photogrammetry-based Framework to Facilitate Image-based Modeling and Automatic Camera Tracking

We propose a framework that extends Blender to exploit Structure from Motion (SfM) and Multi-View Stereo (MVS) techniques for image-based modeling tasks such as sculpting or camera and motion tracking. Applying SfM allows us to determine camera motions without manually defining feature tracks or calibrating the cameras used to capture the image data. With MVS we are able to automatically compute dense scene models, which is not feasible with the built-in tools of Blender. Currently, our framework supports several state-of-the-art SfM and MVS pipelines. The modular system design enables us to integrate further approaches without additional effort. The framework is publicly available as an open source software package.

==> framework_overview_figure.tex <==


\begin{figure*}[!htb]

	\centering
	\begin{tikzpicture}[auto]
	
		% available sizes are:
		% \tiny, \scriptsize, \footnotesize, \small, \normalsize, \large, \Large, \LARGE, \huge, \Huge 
		\newcommand{\figureTextSize}{\small}
	
		% https://tex.stackexchange.com/questions/15028/calculating-right-angle-triangle-side-inside-latex
		% \pgfmathsetmacro and \pgfmathsetlengthmacro can also be defined outside of tikzppicture
		% \pgfmathsetmacro and \pgfmathsetlengthmacro supports floating point numbers
		% \pgfmathsetmacro esults in a numeric output which is void of any unit of measure
		% \pgfmathsetlengthmacro preserves the dimension component
		
		\pgfmathsetlengthmacro{\satImageWidth}{1.1in}
		\pgfmathsetlengthmacro{\satImageWidthHalf}{0.55in}
		\pgfmathsetlengthmacro{\SfMWidth}{1.4in}
		\pgfmathsetlengthmacro{\recWidth}{1.8in}
		
		\pgfmathsetmacro{\colDistance}{4.5}
		\pgfmathsetmacro{\rowDistance}{-2}
		
		\coordinate (fullRow) at (0, \rowDistance);
		\coordinate (fullCol) at (\colDistance, 0);
		
		\coordinate (halfRow) at (0,0.5 * \rowDistance);
		\coordinate (halfCol) at (0.5 * \colDistance, 0);
		
		\coordinate (diagLineOffsetLD) at (-0.25,-0.25);
		\coordinate (diagLineOffsetRD) at (-0.25,0.25);
		
		\pgfmathsetmacro{\firstcol}{0}
		\pgfmathsetmacro{\firstrow}{0}
		
		\pgfmathsetmacro{\secondcol}{\colDistance}
		\pgfmathsetmacro{\secondrow}{\rowDistance + - 2.25}
		
		\pgfmathsetmacro{\thirdcol}{\secondcol + \colDistance}
		\pgfmathsetmacro{\thirdrow}{\secondrow + \rowDistance - 2.25}
	
		\pgfmathsetmacro{\fourthcol}{\thirdcol + \colDistance}
		\pgfmathsetmacro{\fourthrow}{\thirdrow + \rowDistance - 1.75}
		
		\pgfmathsetmacro{\fifthrow}{\fourthrow + \rowDistance}
		
		\pgfmathsetmacro{\sixthrow}{\fifthrow + \rowDistance}
		
		\tikzset{imageStack/.style={
				draw=black, 
				double copy shadow={rotate=60, shadow xshift=0.1cm, shadow yshift=0.1cm}, 
				fill=white, 
				inner sep=0}}
			
		\tikzset{reconstructionResult/.style={inner sep=0}}

		% coordinates are (x,y) = (width, height)
		\coordinate (descr_offset) at (0,1);
	  
 		\node[imageStack] (PAN) at (\firstcol,\firstrow) { 
	  	\includegraphics[ width = \satImageWidth]{14NOV15135121-P1BS-500171606160_05_P005-BROWSE.JPG}};
  	
  		\node (AOI) at ($(\secondcol, \firstrow) + (-1,0)$){ 
  		\includegraphics[ width = \satImageWidth]{aoi_selection_thick.png}};
		
 		\node[imageStack] (MSI) at ($(\thirdcol,\firstrow) + (-2.5, 1)$) { 
		\includegraphics[ width = \satImageWidthHalf]{14NOV15135121-M1BS-500171606160_05_P005-BROWSE.JPG}};

		\node[imageStack] (MSIcropped) at ($(\thirdcol, \firstrow) + (-2.5, -1)$){ 
			\includegraphics[ width = \satImageWidthHalf]{0036_WV03_15DEC11_135506-P1BS-500510591010_01_P001_msi_cropped_resized_25.png}};

		% Second row
		\node[imageStack] (PANcropped) at (\firstcol,\secondrow){ 
			\includegraphics[ width = \satImageWidth]{0036_WV03_15DEC11_135506-P1BS-500510591010_01_P001_pan_cropped_resized_25.png}};
		
		\node[imageStack] (PANSharpenedRes) at (\thirdcol, \secondrow){ 
			\includegraphics[ width = \satImageWidth]{0036_WV03_15DEC11_135506-P1BS-500510591010_01_P001_pan_sharpened_resized_25.png}};
		
		\node[reconstructionResult] (sfm) at ($(\secondcol, \secondrow) - (0, 0.4)$){ 
			\includegraphics[ width = \SfMWidth]{sfm_earth_2_resized_50.png}};
	
		% Third row
 		\node[imageStack] (PANskewCorrected) at (\firstcol,\thirdrow) { 
			\includegraphics[ width = \satImageWidth]{0036_WV03_15DEC11_135506-P1BS-500510591010_01_P001_pan_skew_correction_resized_25.png}};
		
 		\node[reconstructionResult] (mvs) at (\secondcol,\thirdrow) { 
			\includegraphics[ width = \recWidth]{mvs_resized_25.png}};
		
 		\node[imageStack] (MSIskewCorrected) at (\thirdcol,\thirdrow) { 
			\includegraphics[ width = \satImageWidth]{0036_WV03_15DEC11_135506-P1BS-500510591010_01_P001_msi_skew_correction_resized_25.png}};
		

		\node[reconstructionResult] (mesh) at ($(\firstcol, \fourthrow) + (1,0)$){ 
			\includegraphics[ width = \recWidth]{mesh_geometry_resized_25.png}};
		
		\node[reconstructionResult] (texturedMesh) at ($(\thirdcol, \fourthrow) - (1,0)$){ 
			\includegraphics[ width = \recWidth]{mesh_textured_resized_25.png}};

		
	  	\tikzset{arrowStyle/.style={->, line width=0.5mm}}
		\draw[arrowStyle] (AOI) -- (PANcropped);
		\draw[arrowStyle] (AOI) -- (MSIcropped);

		\draw[arrowStyle] (PAN.south west) -- ($(PAN.south west) +(diagLineOffsetLD)$) -- ($(PANcropped.north west) + (diagLineOffsetRD)$) -- (PANcropped.north west);
		\draw[arrowStyle] (MSI) -- (MSIcropped);
		
		% https://tex.stackexchange.com/questions/377618/centre-of-a-tikz-node
		% http://ctan.mirror.norbert-ruehl.de/graphics/pgf/base/doc/pgfmanual.pdf
		\draw[arrowStyle] (PANcropped.north east) -- ($(PANcropped.north east) - (diagLineOffsetLD)$) -- ($(PANSharpenedRes.north west) + (diagLineOffsetRD)$) -- (PANSharpenedRes.north west);
		\draw[arrowStyle] (MSI) -- (MSIcropped);
		
		\draw[arrowStyle] (PANcropped) -- (sfm);
		\draw[arrowStyle] (PANcropped.south west) -- ($(PANcropped.south west) +(diagLineOffsetLD)$) -- ($(PANskewCorrected.north west) + (diagLineOffsetRD)$) -- (PANskewCorrected.north west);
		
		\draw[arrowStyle] (sfm) -- (PANskewCorrected);
		\draw[arrowStyle] (sfm) -- (mvs);
		\draw[arrowStyle] (sfm) -- (MSIskewCorrected);
		\draw[arrowStyle] ($(sfm.10)$) -- ($(sfm.10) + (0.75,0)$) -- (texturedMesh.125);
				
		\draw[arrowStyle] (PANSharpenedRes.south east) -- ($(PANSharpenedRes.south east) -(diagLineOffsetRD)$) -- ($(MSIskewCorrected.north east) - (diagLineOffsetLD)$) -- (MSIskewCorrected.north east);
		
		\draw[arrowStyle] (PANskewCorrected) -- (mvs);
		\draw[arrowStyle] (mvs) -- (mesh);
		\draw[arrowStyle] (MSIcropped) -- (PANSharpenedRes);
		\draw[arrowStyle] (MSIskewCorrected.south east) -- ($(MSIskewCorrected.south east) -(diagLineOffsetRD)$) -- ($(texturedMesh.north east) - (diagLineOffsetLD)$) -- (texturedMesh.north east);

		\tikzset{descrStyle/.style={align=left, font=\figureTextSize}} % fill=white

		\node [descrStyle] at ($(PAN)+(0, 2)$) {PAN Images};
		\node [descrStyle, align=center] at ($(AOI)+(0, 2) $) {Area of Interest \\ (AOI)};
		\node [descrStyle] at ($(MSI)+(0, 1.25) $) {MSI Images};
		
		\node [descrStyle, align=center] at ($(PANcropped)+(0,2.1)$) {AOI Extraction, \\ PAN Tonemapping};
		\node [descrStyle, right] at ($(MSIcropped)+(1,1)$) {AOI Extraction, \\ MSI Tonemapping};
	
		\node [descrStyle, align=center] at ($(PANSharpenedRes)+(0, 2.10)$) {PAN-Sharpening};
		
		\node [descrStyle, align=center] at ($(PANskewCorrected)+(0, 1.95)$) {Skew-correction of \\ Images and Cameras};
		\node [descrStyle, align=center] at ($(MSIskewCorrected)+(0, 1.95)$) {Skew-correction of \\ Images and Cameras};
		
		\node [descrStyle] at ($(sfm)+(0, 1.85)$) {SfM};
		\node [descrStyle, right] at ($(mvs)+(0, 1.75)$) {MVS};

		\node [descrStyle] at ($(mesh)+(0, 1.75)$) {Meshing};
		\node [descrStyle] at ($(texturedMesh)+(0, 1.75)$) {Texturing};

	  \end{tikzpicture}

	\caption{Pipeline components} 
	\label{reconstruction_pipeline}
\end{figure*}

==> framework_verification.tex <==
\subsection{Visualization and Inspection}

\noindent The framework provides several options to visually assess the correctness of the imported results.
\begin{itemize}
	\item Adding background images (see image \figref{fig_background_image}) allows to assess the consistency of the input images and the corresponding projections of the scene geometry, \ie the point cloud or the textured mesh.
	\item 
\end{itemize}
